How Much Does It Cost to Answer My Question? Benchmarking Cloud VLM-based VQA Systems

Vision-language models (VLMs) are becoming a practical backend for mobile visual question answering (VQA) systems, enabling smartphones and smart glasses to answer users' questions about the physical world. Since modern VLMs remain difficult to run on mobile and edge devices, VQA systems increasingly offload inference to cloud-based VLMs. This gives mobile devices access to stronger computation, but it also makes visual input preparation a key system variable: how the image is prepared before offloading affects not only answer quality but also payload size, token cost, and system latency. Proprietary APIs expose little control over model internals or serving behavior, leaving client-side preprocessing as the main practical optimization space for downstream developers. Many such techniques have been proposed for visual offloading, yet their cost-quality impact on commercial cloud VLMs has never been studied. To fill this gap, we present VQABench, the first systematic benchmark that treats client-side input preprocessing as a controlled variable for cloud-VLM-based VQA. We evaluate 12 preprocessing techniques across three VQA datasets and four commercial VLMs from three providers, totaling 95,168 API calls. Our results show that preprocessing is not universally beneficial: its effectiveness depends on the target model, API paradigm, provider token-accounting rule, and task formulation. A poorly selected preprocessing strategy can increase deployment cost or latency while degrading answer accuracy. Overall, our benchmark clarifies when preprocessing helps, when it fails, and why, providing insights to guide future research and real-world deployment of VQA systems.

==> 03Background.tex <==
% % ══════════════════════════════════════════════════════════════════
% \section{Background}\label{sec:background}
% % ══════════════════════════════════════════════════════════════════

% This section provides the technical background needed to interpret the benchmark. We first describe how vision-language models are deployed in cloud-offloaded pipelines. We then introduce the mechanics of the cloud VLM cost chain.  

% ══════════════════════════════════════════════════════════════════
% Subsection: System Pipeline of a Cloud-based VLM Request.
%
% Placement: should appear BEFORE the Cost Chain subsection so the
% pipeline mechanics motivate the cost analysis that follows.
%
% Required macros: \sysname (already defined).
%
% New citations used (most already in existing bib):
%   openai_realtime_websocket_mode (NEW --- BibTeX entry below)
%   openai_vision_docs, anthropic_vision_docs,
%   gemini_image_understanding (already in bib)
%   openai_api_pricing, anthropic_pricing_docs, gemini_pricing
%   (already in bib)
% ══════════════════════════════════════════════════════════════════

% \subsection{System Pipeline of a Cloud-based VLM}
% \label{ssec:bg_pipeline}


% \paragraph{\textbf{REST and Realtime as two API paradigms}.}

% \subsubsection{API Paradigms}
% Commercial VLMs have REST and Realtime as the two APIs paradigms. 

% REST endpoints follow the standard HTTP request--response cycle: the client opens a TLS connection, sends a JSON body containing the image and prompt, and receives either a unary response or a server-sent event stream carrying incremental output tokens~\cite{openai_api_pricing,anthropic_pricing_docs,gemini_pricing}. Each request reopens a seperate connection state. 

% Realtime endpoints use a persistent secure WebSocket with bidirectional event streaming~\cite{openai_realtime_websocket_mode}. After a single handshake, the client and server exchange typed events --- session updates, item appends, response creates, output deltas, completion signals --- over the same socket for as long as the session lives. 

% The trade-off is straightforward.  REST is stateless and operationally simple, but every request pays the cost of connection setup, TLS handshake, and full prompt re-transmission. WebSocket amortises those costs across many turns, but binds session state to a connection the client must hold open. Whether this lowers end-to-end latency depends on payload, network, and request rate.  \sysname{} measures both.

% \paragraph{Image tokenisation is provider-specific.} Each provider converts an image into tokens differently, and the differences are large enough to affect which preprocessing technique is most cost-effective. For instance, OpenAI's GPT-4o-class models resize the image to fit within a $2048^2$ box with the shortest side scaled to $768$\,px, then tile it into $512\!\times\!512$
% patches at $170$ tokens per tile plus an $85$-token base charge~\cite{openai_vision_docs}.  Mini and nano variants use $32\!\times\!32$ patches with a $1{,}536$-patch budget and a model-specific multiplier. Anthropic tokenises approximately as $\lceil w \cdot h / 750 \rceil$ tokens, billing roughly per pixel~\cite{anthropic_vision_docs}. Gemini issues a flat $258$ tokens for images whose longer side is at most $384$\,px; beyond that threshold, it tiles the image at $768\!\times\!768$ and charges $258$ tokens per tile~\cite{gemini_image_understanding}. A $1024\!\times\!1024$ image therefore maps to roughly $765$ tokens on GPT-4o, $\sim{}1{,}400$ tokens on Claude, and $\sim{}1{,}032$ tokens on Gemini --- nearly a $2\times$ spread for the same pixels.  The accounting is also discontinuous: shrinking an image just below a tile boundary collapses its token count, but shrinking it slightly above the boundary does not. A preprocessing technique that is favourable on one provider can be neutral on another and counterproductive on a third, and a single-provider benchmark cannot detect this.

% ── 2.2 ──────────────────────────────────────────────────────────


==> abstract.tex <==
% Vision-language models (VLMs) are becoming the practical backend for mobile visual question answering (VQA) assistants, enabling smartphones and smart glasses to answer users’ questions about the ambient world. Since modern VLMs remain difficult to run on mobile devices, the most capable VQA systems today increasingly rely on cloud-based VLMs. This cloud-centric design gives mobile devices access to stronger computation, but makes each VQA request depend on the visual input sent to the cloud, which affects payload, token usage, system latency, and answer quality. Because traditional token reduction and computation-offloading optimizations require server-side cooperation that proprietary VLMs do not expose, client-side input preprocessing becomes the main practical choice to optimize this cost--quality trade-off. In fact, many client-side preprocessing techniques have been proposed for this purpose. Yet their effectiveness on cloud VLMs remains unclear, as they may affect accuracy, latency, payload, and token usage in different and sometimes conflicting ways. This makes it difficult for application developers to choose the right preprocessing strategy for a given deployment scenario. To fill this gap, we present \sysname, the first systematic benchmark that evaluates 12 preprocessing techniques across three VQA datasets, and four commercial VLMs, totaling 95{,}168 API calls. Overall, our benchmark reveals and explains how preprocessing choices reshape the end-to-end cost--quality trade-off of cloud-VLM-based VQA across four performance dimensions, providing evidence and insights to guide future research and real-world system deployment.

Vision-language models (VLMs) are becoming a practical backend for mobile visual question answering (VQA) systems, enabling smartphones and smart glasses to answer users’ questions about the physical world. Since modern VLMs remain difficult to run on mobile devices, VQA systems increasingly offload inference to cloud-based VLMs. This gives mobile devices access to stronger computation, but it also makes visual input preparation a key system variable: how the image is prepared before offloading affects not only answer quality but also payload size, token cost, and system latency. Proprietary APIs expose little control over model internals or serving behavior, leaving client-side preprocessing as the main practical optimization space for downstream developers. Many such techniques have been proposed for visual offloading, yet their cost–quality impact on commercial cloud VLMs has never been studied. To fill this gap, we present \sysname, the first systematic benchmark that treats client-side input preprocessing as a controlled variable for cloud-VLM-based VQA. We evaluate 12 preprocessing techniques across three VQA datasets and four commercial VLMs from three providers, totaling 95,168 API calls. Our results show that preprocessing is not universally beneficial: its effectiveness depends on the target model, API paradigm, provider token-accounting rule, and task formulation. A poorly selected preprocessing strategy can increase deployment cost or latency while degrading answer accuracy. Overall, our benchmark clarifies when preprocessing helps, when it fails, and why, providing insights to guide future research and real-world deployment of VQA systems. %We make the benchmark artifacts publicly available to support reproducible comparison and future studies: \url{https://anonymous.4open.science/r/VQABench-8181/.}




% Since modern VLMs remain difficult to run on mobile devices, VQA systems increasingly rely on cloud-based VLMs. This cloud-centric design gives mobile devices access to stronger computation, but also turns each VQA request into an offloading problem where the visual input interacts with the cloud VLM pipeline to shape the system’s cost--quality trade-off. Since proprietary APIs expose little control over model internals or serving behavior, client-side input preprocessing is the main optimization space left to downstream developers. Yet, despite the many preprocessing techniques proposed for visual offloading, their cost--quality impact on commercial cloud VLMs remains unclear. 







==> benchmarkbackup.tex <==
% ══════════════════════════════════════════════════════════════════
\section{Benchmark Design}\label{sec:design}
% ══════════════════════════════════════════════════════════════════

Below, we present the design of our benchmarking framework. We first state the research questions and hypotheses that guide the benchmark, then describe the measurement pipeline and instrumentation, the 12~preprocessing techniques, the cloud VLM configurations, the datasets, the planned experiment blocks (\S\ref{ssec:scale}), and finally the evaluation metrics and statistical analysis approach (\S\ref{ssec:metrics}).

% ── 3.1 ──────────────────────────────────────────────────────────
\subsection{Research Questions and Hypotheses}\label{ssec:rqs}

\sysname is designed as a measurement study of \emph{the system as a whole}: the cost landscape of cloud-offloaded multimodal inference and the leverage that input-side optimization provides within that landscape. Our investigation covers a wide range of broader characterization from VLM model choice, provider choice, API paradigm, network conditions, as well as preprocessing techniques. The benchmark is therefore organized around three research questions that move from the system context outward to its input-side levers and finally to overall trade-offs.

% \begin{itemize}[nosep, label=\textbf{RQ\arabic*}]

\begin{itemize}[leftmargin=*]

\item \textbf{RQ1: Cost landscape.}
  What are the dominant cost factors of cloud-offloaded multimodal VLM inference, and how do they vary across models, providers, API paradigms, and network conditions?  In particular, how are the five cost dimensions---payload size, token consumption, monetary cost, end-to-end latency, and task accuracy---related to one another?

\item \textbf{RQ2: Input-side optimization.} Within the cost landscape characterized by RQ1, how does image preprocessing affect each cost dimension?  Which techniques reduce payload, tokens, latency, and monetary cost; what local preprocessing overhead do they introduce on the client; and to what extent do they preserve task accuracy relative to a no-preprocessing baseline?

\item \textbf{RQ3: System-level trade-offs.} Considering the cost landscape (RQ1) and the input-side levers
  (RQ2) jointly, which combinations of model, API, and preprocessing offer the most favorable balance of efficiency and accuracy for interactive cloud-offloaded multimodal inference? How sensitive are the resulting recommendations to question type, network condition, and choice of provider?

\end{itemize}

% \noindent
\textbf{Working hypotheses.} To support quantitative analysis, we evaluate seven working hypotheses that operationalize these questions into specific, testable predictions. %The first three concern the cost landscape itself; the next three concern how preprocessing affects that landscape; the last concerns when region-selective preprocessing succeeds or fails.

\medskip
\noindent\emph{Hypotheses on the cost landscape (RQ1).}

\begin{itemize}[nosep, leftmargin=*]

\item \textbf{H1 (system-level variation).}
  Cloud VLM cost dimensions---latency, payload, token consumption,  and monetary cost---vary substantially across models, providers, and API paradigms.  Model and API selection therefore set the baseline cost regime within which any input-side optimization must operate, and the magnitude of this baseline variation may exceed the variation achievable through preprocessing alone.

\item \textbf{H2 (cost decoupling).}
  The five cost dimensions are decoupled rather than co-varying.
  In particular, payload reduction does not imply proportional
  token reduction, because commercial providers tokenize images
  according to pixel-grid tilings rather than encoded file size.
  This decoupling means that bandwidth optimization (fewer bytes)
  and cost optimization (fewer billable tokens) require
  fundamentally different strategies.

\item \textbf{H3 (API-paradigm dependence).}
  The strength of the payload-to-latency coupling differs between
  API paradigms.  Streaming or Realtime interfaces are likely to
  show stronger latency response to changes in transmitted payload
  than request-response (REST) interfaces, where server-side
  scheduling and per-request overhead may dominate.  The latency
  impact of any input-side optimization is therefore
  API-dependent.

\end{itemize}

\medskip
\noindent\emph{Hypotheses on input-side preprocessing (RQ2).}

\begin{itemize}[nosep, leftmargin=*]

\item \textbf{H4 (preprocessing efficiency).}
  Image preprocessing reduces transmitted payload, token
  consumption, monetary cost, and end-to-end latency relative to
  the no-preprocessing baseline.  The magnitude and direction of
  the effect depend on the technique family: compression primarily
  reduces payload, while region-selective methods primarily affect
  tokens by changing the pixel content seen by the model.  Local
  preprocessing overhead, however, can offset cloud-side gains,
  particularly for compute-heavy methods such as object detection.

\item \textbf{H5 (accuracy preservation).}
  Preprocessing techniques do not preserve task accuracy equally.
  Aggressive global reduction or poorly aligned region selection
  may degrade accuracy below the no-preprocessing baseline, while
  lightweight compression and well-aligned region selection may
  preserve accuracy at near-baseline levels.

\item \textbf{H6 (region-selective Pareto advantage).}
  Region-selective techniques that preserve task-relevant content
  can achieve a more favorable efficiency--accuracy trade-off than
  naive global reduction, because they retain pixel-level detail
  where it matters most while discarding background.  This
  advantage is conditional on the alignment between the selection
  signal (human gaze, algorithmic saliency, or object detection)
  and the visual reasoning required by the task.

\end{itemize}

\medskip
\noindent\emph{Hypothesis on system-level trade-offs (RQ3).}

\begin{itemize}[nosep, leftmargin=*]

\item \textbf{H7 (question-type sensitivity).}
  The benefit of region-selective preprocessing depends on the
  type of question being asked.  Gaze-guided cropping in
  particular may fail on questions requiring global scene
  understanding---counting objects across the image, comparing
  spatially distant elements, or describing overall
  composition---where the relevant information lies outside any
  single attended region.  A complete trade-off analysis must
  therefore condition on question type rather than reporting only
  aggregate accuracy.

\end{itemize}

\medskip
\noindent\textbf{Mapping between hypotheses and research questions.}
H1--H3 are tested in the cost-landscape characterization
(\S\ref{ssec:context}), which evaluates the baseline configuration
across models, providers, API paradigms, and network conditions
before any preprocessing is applied.  H4--H6 are tested in the
preprocessing evaluation
(\S\ref{ssec:efficiency}--\S\ref{ssec:accuracy}), which compares
the 12~techniques on efficiency and accuracy.  H7 is addressed by
the Pareto and question-type analyses
(\S\ref{ssec:pareto}, \S\ref{ssec:discussion}), which condition the
trade-off recommendations on question category and dataset.

This organization reflects the broader scope of the benchmark.
Rather than treating preprocessing as the sole object of study, we
treat it as one input-side lever evaluated within an explicitly
characterized system context.  The reader can therefore interpret
each finding either as a property of preprocessing in isolation or
as a property of the joint system---model, API, network, and
input---in which preprocessing operates.


% ── 3.2 ──────────────────────────────────────────────────────────
\subsection{Pipeline Architecture and Instrumentation}
\label{ssec:pipeline}

Figure~\ref{fig:pipeline} shows the \sysname pipeline. For each image-question sample, the local client loads the sample from a unified prepared dataset, applies one preprocessing technique, encodes the result as a Base64 JSON payload, transmits it to the cloud VLM, receives the streamed response, extracts the textual answer, and logs all metrics. This process is repeated for every technique on the same sample, implementing the paired design described in \S\ref{ssec:datasets}.

\begin{figure}[t]
  \centering
  \fbox{\parbox{0.95\columnwidth}{\centering\vspace{2.5em}%
    \small
    Raw image $\xrightarrow{\texttt{preprocess\_ms}}$
    Processed image $\xrightarrow{\text{Base64 encode}}$\\
    JSON payload $\xrightarrow{\texttt{upload\_ms}}$
    Cloud VLM $\xrightarrow{\texttt{stream\_ms}}$
    Answer + metrics\\[0.6em]
    \footnotesize
    \textbf{Above the dashed line (hardware-dependent):}
    local preprocessing time.\\
    \textbf{Below the dashed line (hardware-independent):}
    tokens, cost, accuracy, API latency.
    \\[2em]}}
  \caption{\sysname measurement pipeline.  Metrics below the
  dashed line depend only on the bytes that arrive at the
  cloud server; they are therefore independent of the client
  device.  Local preprocessing time above the dashed line
  depends on the specific hardware used to run the technique.}
  \label{fig:pipeline}
\end{figure}

\paragraph{Benchmark metrics.} We explicitly consider two groups of performance metrics according to whether
they depend on the cloud-hosted LLM server or the mobile client device. 

\textbf{\emph{Server-side metrics}} include token counts, monetary cost, task accuracy, and API latency measured from request transmission to response completion. These metrics are determined entirely by the inputs that arrive at the particular server: an identical Base64-encoded payload should produce identical tokens, identical model responses, and identical cost regardless of whether it was sent from a laptop, a smartphone, a wearable, or a headset. Server-side metrics are therefore \emph{client-independent} and the conclusions drawn from them apply directly to any deployment platform.

\emph{Local preprocessing time} (\texttt{preprocess\_ms}) is the only metric that depends on the client device.  It reflects the computational cost of executing a particular preprocessing technique on the specific hardware used to run it.  By measuring and reporting the two groups separately, the benchmark allows cloud-side conclusions to generalize across devices while local preprocessing overhead can be interpreted as a device-specific lower or upper bound.  On weaker edge hardware than the laptop used in our experiments, local overhead would be proportionally larger; on stronger hardware it would be smaller.

\paragraph{Latency decomposition.}
We decompose end-to-end latency into client-observable stages without requiring access to provider internals.  The four fundamental stages are:

\begin{itemize}[nosep, leftmargin=*]
\item \texttt{preprocess\_ms}: the wall-clock time to execute
  the preprocessing technique on the client device
  (hardware-dependent).
\item \texttt{request\_upload\_ms}: the time to transmit the
  Base64-encoded JSON payload to the provider's API endpoint.
\item \texttt{request\_to\_first\_response\_ms}: the time from
  upload completion to receiving the first streamed response
  event from the model, capturing both server-side queueing
  and the start of inference.
\item \texttt{first\_response\_to\_done\_ms}: the time to
  receive the complete streamed response after the first
  response event.
\end{itemize}

Two aggregate metrics are derived from these stages.
\texttt{end\_to\_end\_ms} measures the full cloud-side API
interaction from request initiation to response completion;
it is hardware-independent once the transmitted payload is
fixed.  \texttt{total\_pipeline\_ms} additionally includes
the local preprocessing time:
\begin{equation}
  \texttt{total\_pipeline\_ms} = \texttt{preprocess\_ms} +
  \texttt{end\_to\_end\_ms}.
  \label{eq:pipeline}
\end{equation}
This distinction is important because a preprocessing
technique may reduce cloud-side latency while simultaneously
increasing total pipeline time if its local computation is
expensive.  A complete picture of system-level performance
requires both metrics.

For experiments using the OpenAI Realtime WebSocket API,
finer-grained latency decomposition is available because the
streaming protocol exposes intermediate events.  We additionally
log request creation time, send-to-first-server-event,
first-server-event-to-first-token, and first-token-to-done.
Connection acquisition and session-update costs are recorded
separately so that per-request latency is not conflated with
one-time setup overhead.

\paragraph{Logging granularity.}
Each request produces a structured log record with more than
35~fields.  These cover absolute and relative timestamps for
each pipeline stage, original and processed pixel dimensions,
multiple representations of payload size (raw binary bytes,
Base64-encoded bytes, full JSON envelope size including text
prompt and metadata), compression ratio relative to the
original image, all latency stages described above, provider-
reported token counts (text input, image input, output,
cached, total), estimated monetary cost in USD computed from
active provider pricing, and task accuracy as measured by the
applicable evaluation metric.  Logging at this granularity
allows post-hoc analysis to identify which specific component
of the pipeline contributes to observed differences.

\paragraph{Extensibility.}
Adding a new preprocessing technique to the benchmark requires
implementing a single Python function that accepts an image
and gaze trace (if applicable) and returns the processed
image.  Adding a new provider requires implementing a request
formatter and response parser specific to that provider's API
contract.  The measurement harness, metrics computation, and
logging format remain unchanged across techniques and
providers.


% ── 3.3 ──────────────────────────────────────────────────────────
\subsection{Preprocessing Techniques}\label{ssec:techniques}

We evaluate 12~preprocessing techniques organized into three
families (Table~\ref{tab:techniques}), selected to span both
global reduction methods that modify the entire image and
region-selective methods that preserve task-relevant content
while discarding background.  Each region-selective method has
two variants: a \emph{crop-only} variant that transmits only
the selected region, and a \emph{+T} variant that additionally
includes a $28{\times}28$ global thumbnail to preserve coarse
scene context for questions requiring global understanding.

\begin{table}[t]
\centering
\caption{Preprocessing techniques evaluated in \sysname.
\emph{+T} variants include a $28{\times}28$ global-context
thumbnail in addition to the primary region.  All processed
outputs are JPEG-encoded at quality~85 before transmission
unless otherwise noted.}
\label{tab:techniques}
\small
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Family} & \textbf{ID} & \textbf{Method}
  & \textbf{Selection signal} \\
\midrule
Baseline    & B0 & Baseline\_NoOp                & --   \\
\midrule
\multirow{3}{*}{\makecell[l]{Global\\reduction}}
  & G1 & Downsampler $100{\times}100$            & --   \\
  & G2 & GlobalThumbOnly $28{\times}28$          & --   \\
  & G3 & Grayscale                               & --   \\
\midrule
\multirow{2}{*}{Compression}
  & C1 & JPEG\_Q85                               & --   \\
  & C2 & WebP\_Q85                               & --   \\
\midrule
\multirow{2}{*}{\makecell[l]{Gaze-guided\\ROI}}
  & R1 & GazeROI                                 & Gaze \\
  & R2 & GazeROI+T                               & Gaze \\
\midrule
\multirow{2}{*}{\makecell[l]{Saliency-based\\ROI}}
  & R3 & SalientROI                              & Auto \\
  & R4 & SalientROI+T                            & Auto \\
\midrule
\multirow{2}{*}{\makecell[l]{Object-detection\\ROI}}
  & R5 & YOLOv12ROI                              & Auto \\
  & R6 & YOLOv12ROI+T                            & Auto \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Global reduction.}
\textbf{Downsampler} uniformly resizes the image to
$100{\times}100$ pixels.  This is the simplest global
simplification strategy and serves as a reference for how
much information loss is acceptable when applied
uniformly~\cite{Talebi2021}.
\textbf{GlobalThumbOnly} reduces the image to an extreme
$28{\times}28$ thumbnail, serving as an empirical lower
bound on how much visual content can be discarded before
task accuracy degrades severely.
\textbf{Grayscale} converts the RGB image to a single
luminance channel, testing whether removing chromatic
information reduces payload or tokens while preserving
sufficient task-relevant content~\cite{kanan2012grayscale}.

\paragraph{Compression.}
\textbf{JPEG\_Q85} applies lossy JPEG compression at
quality~85, a long-standing standard for image
transmission~\cite{wallace1991jpeg}.
\textbf{WebP\_Q85} applies lossy WebP compression at the
same quality level, providing a modern alternative that
generally achieves stronger compression at comparable
perceptual quality~\cite{ginesu2012webp}.  Both formats are
natively accepted as image inputs by all three evaluated
providers.

\paragraph{Region-selective methods.}
\textbf{GazeROI} uses human gaze coordinates from dataset
annotations to define a region of interest centered on the
user's attended area, approximating foveated visual
processing~\cite{Chen2025}.  The gaze-driven cropping is
parameterized by $\rho{=}0.5$ (relative crop radius
coefficient), a minimum relative ROI size of~0.2, Gaussian
smoothing with $\sigma{=}15.0$ applied to the gaze heatmap,
and an ROI detection size of~64 pixels at the analysis stage.
Gaze coordinates are drawn from offline dataset annotations
rather than from a live eye tracker; this should therefore be
interpreted as an offline proxy for gaze-informed interactive
deployment.

\textbf{SalientROI} uses a spectral-residual saliency
detector to identify visually prominent regions without any
human input~\cite{saliencyDetection}.  The method computes
the Fourier spectrum at analysis size~64, applies a
$3{\times}3$ average filter for spectral residual estimation,
and selects regions where saliency exceeds
$3.0{\cdot}\mathbb{E}[S(x)]$, with the resulting region map
smoothed using $\sigma{=}8.0$.  This represents a fully
automatic alternative to gaze-based selection.

\textbf{YOLOv12ROI} uses YOLOv12 object detections (ONNX
runtime, \texttt{yolo12n} model, input resolution~640,
confidence threshold~0.25, IoU threshold~0.45) to extract
semantically meaningful entities.  When multiple objects are
detected, separate crops are transmitted, so the combined
payload can exceed the original
image~\cite{benchmarkingNeuralNets}.  YOLOv12 also introduces
non-trivial local CPU inference overhead.  This overhead is
hardware-dependent and would be substantially larger on
edge-class hardware than on the laptop used in our
experiments.


% ── 3.4 ──────────────────────────────────────────────────────────
\subsection{Models and Providers}\label{ssec:models}

We evaluate four cloud VLM configurations spanning three
commercial providers and two API paradigms
(Table~\ref{tab:models}).  These configurations were chosen
through a separate model screening phase
(13~candidate models, 100~baseline VQA-MHUG samples each), the
results of which are presented in \S\ref{ssec:context}.

\begin{table}[t]
\centering
\caption{Cloud VLM configurations used in the main experiments.}
\label{tab:models}
\small
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Provider} & \textbf{Model} & \textbf{API}
  & \textbf{Role in experiments} \\
\midrule
OpenAI    & gpt-realtime-mini & WebSocket
  & Primary model \\
OpenAI    & gpt-5.4           & REST
  & REST comparison \\
Anthropic & Claude Sonnet 4.6 & REST
  & Cross-provider check \\
Google    & Gemini 3 Flash    & REST
  & Cross-provider check \\
\bottomrule
\end{tabular}
\end{table}

\textbf{gpt-realtime-mini} (OpenAI Realtime API) serves as the
primary model for the main experiments.  Its low-latency
WebSocket serving is the closest available proxy for
interactive deployment, where the cloud must respond within
a few hundred milliseconds for a multimodal assistant to feel
responsive.  Although stronger models exist on REST APIs at
higher accuracy, their substantially higher latency makes
them less representative of interactive use.

\textbf{gpt-5.4} (OpenAI REST API) provides a higher-accuracy
comparison point on the same provider, allowing us to isolate
the effect of API paradigm (Realtime WebSocket vs.\ REST) from
the effect of provider.

\textbf{Claude Sonnet 4.6} (Anthropic) and \textbf{Gemini 3
Flash} (Google) serve as cross-provider robustness checks on
a shared subset of 500~VQA-MHUG samples.  These experiments
test whether the relative ordering of preprocessing
techniques observed on OpenAI generalizes to other commercial
VLM providers.


% ── 3.5 ──────────────────────────────────────────────────────────
\subsection{Datasets}\label{ssec:datasets}

No single public dataset captures all aspects of gaze-enabled
multimodal interaction.  We therefore use three datasets with
distinct, complementary roles (Table~\ref{tab:datasets}).
These are not aggregated into a single combined score; each
dataset is evaluated within its intended task setting and
reported separately.

\begin{table}[t]
\centering
\caption{Datasets used in \sysname and their roles in the
evaluation.}
\label{tab:datasets}
\small
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{@{}llclr@{}}
\toprule
\textbf{Dataset} & \textbf{Role} & \textbf{Gaze}
  & \textbf{Accuracy metric} & \textbf{$N$} \\
\midrule
VQA-MHUG~\cite{VQA-MHUG}
  & Primary
  & \checkmark
  & VQA soft acc.
  & 3{,}990 \\
DriVQA~\cite{DriVQA}
  & Driving case study
  & \checkmark
  & LLM judge
  & 24 \\
VOILA-A~\cite{voilaA}
  & Open-ended ext.
  & Proxy
  & LLM judge
  & 500 \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{VQA-MHUG (primary benchmark).}
VQA-MHUG~\cite{VQA-MHUG, balanced_vqav2} contains 11{,}970
gaze samples across 3{,}990 question-image pairs drawn from
the VQAv2 validation set.  Each sample consists of an image,
a natural-language question, ten human reference answers, and
gaze recordings from 49~participants.  This combination
supports both gaze-guided and non-gaze preprocessing
techniques on the same samples, making it ideal as the
primary quantitative benchmark.  Accuracy is measured using
standard VQA soft accuracy, $\min(m/3,\,1)$, where $m$ is
the number of matching human reference answers.

\paragraph{DriVQA (driving-scenario case study).}
DriVQA~\cite{DriVQA} provides 24~driving-scenario questions
with gaze data recorded from 34~participants using a
Tobii Pro X3-120 eye tracker.  Each sample has
approximately 66--68 human reference answers merged across
two test sets.  Because of its small size, DriVQA results
have limited statistical power and we interpret them
descriptively as a real-world case study rather than as a
formal statistical benchmark.  Its inclusion allows us to
examine whether preprocessing trends observed on
general-purpose VQA-MHUG hold in a more domain-specific
context.

\paragraph{VOILA-A (open-ended assistance extension).}
VOILA-A~\cite{voilaA} extends evaluation toward open-ended
gaze-conditioned visual assistance, where the model produces
longer natural-language responses rather than short
factual answers.  Mouse traces serve as a scalable proxy for
gaze.  We curated a subset of 500~samples from VOILA-COCO
through manual inspection: 695~candidate samples were
examined and 500~retained after filtering for clarity of the
expected answer.  This curation was performed before
comparing preprocessing outputs to avoid bias.  Open-ended
responses are evaluated using an LLM judge, scored on
evidence consistency, coverage, detail quality, and
unsupported-claim control.

\paragraph{Paired design.}
All three datasets are converted into a unified prepared
format compatible with the measurement pipeline.  Sample
identity is fixed across all 12~preprocessing conditions:
the same image-question pair is processed by every
technique.  For gaze-based techniques, one gaze trace per
sample is selected randomly with a fixed deterministic seed
and held constant across all conditions.  This preserves the
paired structure of the experiment and ensures that observed
differences between techniques are attributable to the
preprocessing method itself rather than to sample-level or
gaze-trace variation.


% ── 3.6 ──────────────────────────────────────────────────────────
\subsection{Experiment Scale and Protocol}\label{ssec:scale}

Table~\ref{tab:blocks} lists the planned experiment blocks
that constitute the full benchmark.  The VQA-MHUG sample
subsets are nested: the 500-sample cross-provider sets
(Anthropic, Gemini) are contained within the 1{,}000-sample
Realtime set, which is itself contained within the
3{,}990-sample REST set.  This nesting preserves the paired
structure across experiment blocks: results on the smaller
subsets are directly comparable to results on the larger
sets.

\begin{table}[t]
\centering
\caption{Planned experiment blocks and sample sizes.  Each
block evaluates all 12~preprocessing techniques on the
specified sample set.}
\label{tab:blocks}
\small
\renewcommand{\arraystretch}{1.06}
\begin{tabular}{@{}llrr@{}}
\toprule
\textbf{Block} & \textbf{Model} & \textbf{$N$} & \textbf{Calls} \\
\midrule
VQA-MHUG Realtime  & gpt-realtime-mini & 1{,}000 & 12{,}000 \\
VQA-MHUG REST      & gpt-5.4           & 3{,}990 & 47{,}880 \\
VQA-MHUG Anthropic & Claude Sonnet 4.6 & 500     & 6{,}000  \\
VQA-MHUG Gemini    & Gemini 3 Flash    & 500     & 6{,}000  \\
DriVQA case study  & gpt-realtime-mini & 24      & 288      \\
VOILA-A extension  & gpt-realtime-mini & 500     & 6{,}000  \\
Repeatability      & gpt-realtime-mini & 50      & 6{,}000  \\
Network (3 cond.)  & gpt-realtime-mini & 100     & 3{,}600  \\
Model screening    & 13 models         & 100     & 1{,}300  \\
\midrule
\multicolumn{3}{@{}l}{+ VOILA-A LLM judge calls}    & 17{,}000 \\
\midrule
\multicolumn{3}{@{}l}{\textbf{Grand total}}          & \textbf{95{,}168} \\
\bottomrule
\end{tabular}
\end{table}

\paragraph{Execution protocol.}
Each block follows a preprocessor-major execution order: the
outer loop iterates over the 12~preprocessing techniques and
the inner loop iterates over the samples within the block.
This ordering ensures that any temporal variation in cloud
serving conditions (server load, network jitter) is
distributed across techniques rather than concentrated on
one technique.  Requests are issued sequentially with retry
handling: up to 8~outer retries with exponential backoff are
attempted before a request is marked as failed and excluded
from the logged record.  Only successful final calls are
logged.

The \textbf{repeatability experiment} repeats the full
12-technique evaluation on 50~fixed samples for 10~independent
runs (6{,}000 calls).  This isolates run-to-run variance from
inter-technique differences and supports distribution-aware
reporting of latency variability.

The \textbf{network-condition experiment} repeats a 100-sample
evaluation under three network conditions (Ethernet, Wi-Fi,
4G mobile) to test whether the relative ranking of
preprocessing techniques is sensitive to connectivity.

\paragraph{Hardware and network.}
All experiments are executed on a single fixed laptop (Intel
Core i7-8750H @ 2.2\,GHz, 16\,GB RAM, NVIDIA GTX~1060 6\,GB,
Windows~11) connected to the TU~Delft network over a
1\,Gbps Ethernet link, except for the explicit
network-condition experiment which additionally evaluates
Wi-Fi and 4G.  YOLOv12 inference runs via ONNX runtime on
CPUExecutionProvider.  Cloud-side metrics are
hardware-independent by construction; local preprocessing
times should therefore be interpreted as a lower bound for
weaker edge-class hardware.


% ── 3.7 ──────────────────────────────────────────────────────────
\subsection{Evaluation Metrics and Statistical Analysis}
\label{ssec:metrics}

Five metric groups are measured jointly for every request.

\begin{enumerate}[nosep, leftmargin=*]
\item \textbf{Latency.} \texttt{preprocess\_ms}
  (hardware-dependent), \texttt{end\_to\_end\_ms} (the full
  cloud-side API interaction; hardware-independent once the
  payload is fixed), and \texttt{total\_pipeline\_ms} (the sum
  of the two).  Decomposed upload, server-wait, and
  response-streaming sub-stages are recorded for finer-grained
  analysis, with additional Realtime-specific stages where
  applicable.
\item \textbf{Payload.} Processed binary bytes, Base64-encoded
  bytes, compression ratio relative to the original image,
  and full JSON envelope size including the text prompt and
  metadata.
\item \textbf{Tokens.} Provider-reported counts for text input
  tokens, image input tokens, output tokens, cached tokens,
  and total tokens.
\item \textbf{Cost.} Per-request monetary cost in USD,
  estimated from the provider-reported token usage and the
  active pricing schedule at the time of the experiment.
\item \textbf{Accuracy.} VQA soft accuracy
  $\min(m/3,\,1)$~\cite{balanced_vqav2} for VQA-MHUG, where
  $m$ is the number of matching human reference answers.
  For DriVQA and VOILA-A, an LLM judge produces graded
  scores~\cite{voilaA}.
\end{enumerate}

\paragraph{Statistical analysis.}
Because each preprocessing technique is evaluated on the same
set of samples within each block, all comparisons are
\emph{paired}.  Each technique is compared against the
no-preprocessing baseline (Baseline\_NoOp) using
baseline-relative percentage reductions for efficiency
metrics and absolute percentage-point changes for accuracy.
Uncertainty is reported through bootstrap confidence
intervals (2{,}000 resamples, 99\% level) for means and
percentiles.  Distribution-aware summaries (median,
inter-quartile range, p90, p95, p99) and cumulative
distribution functions serve as the primary visualizations
for latency, which is right-skewed and affected by
server-side and network variability.  Results emphasize
effect sizes and confidence intervals rather than formal
null-hypothesis significance tests, following standard
practice in measurement studies of cloud and edge
systems~\cite{Lones2024,
semmelrock2023reproducibilitymachinelearningdrivenresearch}.
